Orbital Dynamics at Atmospheric Pressure in a Lensed, Dual-beam, Optical Trap

Orbital optical trapping of a dielectric micro-particle in air was studied experimentally using a lensed, counter-propagating dual-beam trap, and by numerical simulations employing ray optics. The essential attributes of particle dynamics are evaluated as functions of the transverse offset between the beams, the axial offset between the laser foci and the total laser power, both experimentally and computationally. We find that the Q-factor of the orbital motion in this previously unexplored scheme is at least two orders of magnitude higher than values attainable with conventional trapping. Under our experimental conditions, silica micro-spheres orbit up to a maximum frequency of ~2 kHz at atmospheric pressure, which can be further increased by increasing the optical power in the trap. With the help of simulations, we discuss how the experimental technique presented here can be further modified to enhance the Q factor of particle's orbital motion. The evolution of orbital frequencies can be a useful signature in analyzing the kinetics of deposition or loss of materials from the surface of levitated particles in a controlled environment. Hence, the approach reported here could find application as an \emph{in situ} single particle technique for probing reactions relevant to atmospheric chemistry.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
